Transferring Clinical Knowledge into ECGs Representation

Deep learning models have shown high accuracy in classifying electrocardiograms (ECGs), but their black box nature hinders clinical adoption due to a lack of trust and interpretability. To address this, we propose a novel three-stage training paradigm that transfers knowledge from multimodal clinical data (laboratory exams, vitals, biometrics) into a powerful, yet unimodal, ECG encoder. We employ a self-supervised, joint-embedding pre-training stage to create an ECG representation that is enriched with contextual clinical information, while only requiring the ECG signal at inference time. Furthermore, as an indirect way to explain the model's output we train it to also predict associated laboratory abnormalities directly from the ECG embedding. Evaluated on the MIMIC-IV-ECG dataset, our model outperforms a standard signal-only baseline in multi-label diagnosis classification and successfully bridges a substantial portion of the performance gap to a fully multimodal model that requires all data at inference. Our work demonstrates a practical and effective method for creating more accurate and trustworthy ECG classification models. By converting abstract predictions into physiologically grounded \emph{explanations}, our approach offers a promising path toward the safer integration of AI into clinical workflows.

==> papel/experiments.tex <==
\section{Experiments}
% should present the results of both diagnoses classification and lab abnormality estimation, we use the same experiment setup as \cite{alcaraz2025enhancing}

We evaluate our proposed joint-embedding and reconstruction learning paradigm on two distinct downstream tasks: multi-label diagnosis classification; and, laboratory abnormality prediction. To conduct this evaluation, our study utilizes the MIMIC-IV-ECG dataset, a large, publicly available resource uniquely suited for our multimodal research. It contains over 200,000 12-lead electrocardiograms from patients admitted to the Beth Israel Deaconess Medical Center, with a critical linkage to the rich clinical data within the main MIMIC-IV database \citep{johnson2023mimic}. This linkage provides access to a comprehensive set of corresponding tabular data for each ECG, including: (i) laboratory test results; (ii) vital signs and biometrics; and, (iii) ICD-coded discharge diagnoses. The availability of synchronously recorded signals and comprehensive clinical context is fundamental to our approach, as it enables the self-supervised pre-training and provides the ground-truth labels for our downstream tasks. Following established prior work, our experiments focus on the subset of data originating from the emergency department to reflect a challenging and practical clinical screening scenario \citep{strodthoff2024prospects}. Our experimental setup, including data splits, backbone architecture, and evaluation algorithms, rigorously follows the protocol established in \citet{alcaraz2025enhancing} to ensure a fair comparison with all baselines. For the purpose of the lab prediction task, we discriminate the tabular data into two types: the valuable laboratory exam values; and the remaining tabular features, which we term routine clinical data (biometrics and vital signs). All results are reported as the macro-averaged Area Under the Receiver Operating Curve (AUROC) on the held-out test set.

Our primary results are summarized in Table~\ref{tab:results}. We compare our approach against three key baselines as they evaluated in the same dataset:
\begin{enumerate}
    \item \textbf{Supervised Signal-Only \citep{strodthoff2024prospects}:} A model trained for diagnosis classification using only ECG waveforms, representing the standard unimodal baseline;
    \item \textbf{Multimodal Lab Prediction \citep{alcaraz2024cardiolab}:} A model trained to predict lab abnormalities using both ECG and routine clinical data (demographics, vitals), representing the baseline for the reconstruction task;
    \item \textbf{Multimodal Classification \citep{alcaraz2025enhancing}:} A powerful late-fusion model that uses ECG, routine clinical data, and lab values during training and inference to achieve state-of-the-art diagnosis classification. This serves as a practical "upper bound" for performance.
\end{enumerate}

\begin{table*}[t]
\caption{Main results comparing our joint-embedding (JE) and reconstruction approach to established baselines. Filled circles ($\bullet$) indicate a data requirement, while empty circles ($\circ$) indicate it is not required.} % change the symbols
\label{tab:results}
\centering
\resizebox{\textwidth}{!}{ % idk if they enforce the font size
\begin{tabular}{@{}l cc ccc ccc@{}}
\toprule
& \multicolumn{2}{c}{\textbf{Evaluation}} & \multicolumn{3}{c}{\textbf{Inference Requirement}} & \multicolumn{3}{c}{\textbf{Training Requirement}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-6} \cmidrule(lr){7-9}
\textbf{Model} & \textbf{Diagnoses} & \textbf{Lab} & \textbf{Routine} & \textbf{Lab} & \textbf{Diagnoses} & \textbf{Routine} & \textbf{Lab} & \textbf{Diagnoses} \\
\midrule
Supervised Signal-Only & 0.768 & - & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\circ$ & $\bullet$ \\
Multimodal Lab Prediction & - & \textbf{0.762} & $\bullet$ & $\circ$ & $\circ$ & $\bullet$ & $\bullet$ & $\circ$ \\
Multimodal Classification & \textbf{0.826} & - & $\bullet$ & $\bullet$ & $\circ$ & $\bullet$ & $\bullet$ & $\bullet$ \\
\midrule
\textbf{JE + Reconstruction} & 0.795 & 0.701 & \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\circ$} & \textbf{$\bullet$} & \textbf{$\bullet$} & \textbf{$\bullet$} \\
\bottomrule
\end{tabular}
}
\end{table*}

The results suggest the effectiveness of our approach. Our final model, which operates using only the ECG signal at inference time, achieves a classification performance improvement over the signal-only baseline indicating the presence of tabular data knowledge transfer. While it does not reach the performance of the multimodal upper bound which requires full access to all data at test time, our method successfully bridges a significant portion of this performance gap without sacrificing the practicality of unimodal deployment.

Furthermore, we also assess the explanations by evaluating its performance on the laboratory abnormality prediction task. Our approach achieves similar performance to its correspondence baseline, again we treat them as an upper bound because of the data requirement at inference. 


==> papel/introduction.tex <==
\section{Introduction}

% brief introduction of ecg exams, their importance (cardiovascular diseases remain the leading cause of global mortality \cite{roth2017global}) and automatic classification with deep learning
Electrocardiogram (ECG) exams are a fundamental diagnostic tool in medical practice, recording the heart's electrical activity to detect a wide range of cardiovascular conditions \citep{braunwald2015braunwald}. Their importance is substantial, especially considering that cardiovascular diseases remain the leading cause of global mortality \citep{roth2020global}. With the advancement of artificial intelligence, the automatic classification of ECG exams using deep learning techniques has shown remarkable potential \citep{liu2021deep,petmezas2022state}, offering high precision in identifying abnormalities and extracting complex information that can aid in diagnosis.

% then talk about how practitioners don't trust/use healthcare deep learning models, despite their significantly performance, for lack of explainability
Despite the promising performance and significant accuracy achieved by deep learning models in healthcare, their adoption and trust among healthcare professionals remain a challenge \citep{reyes2020interpretability,adeniran2024explainable}. The main barrier to integrating these models into clinical practice lies in their black box nature—the lack of explainability and transparency about how decisions are made \citep{rosenbacke2024explainable}. Physicians, accustomed to clinical reasoning based on evidence and causality, hesitate to trust systems whose internal processes are opaque, leading to mistrust and uncertainty regarding the safety and justification of the predictions \citep{koccak2025bias}.

% this one we change to multimodal in general
% now discuss how explations are often in the form of heatmaps in the input space but physicians dont like them as well, and how text based explanations are better for healthcare
Frequently, the explanations provided by deep learning models are presented as saliency maps, which highlight regions in the input space most relevant to the model's prediction \citep{chaddad2023survey}. However, these heatmaps often fail to bridge the trust gap. Their limitations include a lack of robustness and a frequent misalignment with clinically relevant concepts, making their interpretation ambiguous for diagnostic reasoning \citep{borys2023explainable,zhang2023revisiting}. In contrast, explanations that are grounded in the established clinical lexicon—such as concrete physiological abnormalities—are far more valuable, as they align with the workflow of professionals who rely on structured data like laboratory results to make decisions \citep{hulsen2023explainable,gupta2024comparative}.

% not text supervision
% and finally present multimodal training with text supervision as an approach to handle this problem
To address this explainability gap, we propose a novel multimodal training architecture that enriches an ECG model with knowledge from associated tabular clinical data. Instead of requiring all data modalities at inference, our approach uses a self-supervised, joint-embedding objective to transfer the rich context from laboratory values, vitals, and biometrics into a powerful, unimodal ECG encoder. This enriched encoder is not only more accurate but also inherently more interpretable. By training it to perform a secondary task of predicting lab abnormalities from the ECG signal alone, we create a system that can explain its diagnostic reasoning in terms of concrete, clinically relevant concepts.

In summary, we make the following contribution:
\begin{itemize}
    % \item joint-embedding to distill other-mode knowledge in ecg classification
    \item We propose a joint-embedding pre-training framework to transfer knowledge from multimodal tabular data into a unimodal ECG encoder for the task of diagnosis classification;
    % \item reconstruction of other modes as a alternative to explain automatic diagnoses from ecg
    \item We introduce the prediction of laboratory abnormalities from the ECG embedding as a novel, clinically-grounded method for a indirect explanation of the model's diagnostic outputs.
\end{itemize}


==> short/discussion.tex <==
\section{Conclusion}
In this work, we introduced a novel training paradigm that creates a powerful, practical, and interpretable ECG-based diagnostic model. Our primary contribution is demonstrating that a self-supervised, joint-embedding objective can effectively transfer knowledge from multimodal clinical data into a unimodal encoder, retaining the practical advantage of requiring only the ECG at inference time. Furthermore, we established a new mechanism for model interpretability by predicting associated laboratory abnormalities from the same latent representation, offering a more intuitive alternative to input-space heatmaps. A key limitation is the risk of catastrophic forgetting in our sequential training, which we mitigated by freezing early layers; future work could explore advanced continual learning techniques, a detailed discussion is provided in the Appendix. We also plan to expand our framework to include unstructured text. By converting abstract predictions into physiologically grounded explanations, our approach offers a promising path toward the safer integration of AI into clinical workflows.


==> short/limitations.tex <==
\section{Limitations}
% should discuss the limitations and conclude

% \paragraph{three stage sequential training} this is arguably the main limitation, because of the sequential learning the model could 'forget' the knowledge from the previous training stage. we've tried to train jointly but it was very hard to optimize the three losses. we try to prevent this by partially freezing the earlier layers of the signal encoder. a regularization with label from the previous training might as well be a good solution.
\paragraph{Sequential Training Paradigm} A primary limitation of our work lies in the three-stage sequential training paradigm. This approach introduces the risk of catastrophic forgetting \citep{mccloskey1989catastrophic}, where the model may lose some of the rich, transferred knowledge from the pre-training stage during subsequent finetuning. While a joint, multi-task learning approach was considered, we found the simultaneous optimization of the three distinct loss functions to be highly challenging and unstable. To mitigate this, we partially froze the early layers of the signal encoder, preserving the foundational representations learned during pre-training. Future work could explore more advanced techniques, such as using the transferred representations as a regularization target during the classification phase, to more explicitly retain the pre-trained knowledge. Or training a standard multimodal \emph{all-modes required} model and later train another similar signal encoder to replicate the representation of the former, given that it encodes knowledge from the other modes.

% \paragraph{explanation evaluation} we evaluate our explanation with the performance on the estimation task, however this is assessment is indirect. we didn't evaluate the causal relationships between the lab abnormalities and diagnoses, neither indicate which of them are related to the practitioner.
\paragraph{Evaluation of Explanations} Our evaluation of the model's interpretability is indirect. We use performance on the laboratory abnormality prediction task as a proxy for the quality of the explanation, demonstrating that the ECG embedding contains physiologically relevant information. However, this assessment does not establish a causal relationship between the predicted abnormalities and the final diagnoses, nor does it explicitly highlight which specific abnormalities are most salient for a given diagnostic prediction from the clinician's perspective. The model learns strong correlations, but further investigation, potentially involving causal inference methods or direct clinician feedback studies, would be required to untangle these into clinically actionable insights.

% \paragraph{multimodal learning} when we chose the joint-embedding loss function we select the ones that could be later generalized to a other modes then just the tabular data, in especial the text data. the mimic-iv also has text information with rich information that arguably could improve even more the classification task. also a text-like prediction as explanation is even better than the lab abnormalities one. we plan to incorporate the text in a future work generalizing the joint-embedding loss function to align the embedding of all modes to the signal one. we think keeping one latent representation as an refenrence, or anchor, scale better than the sum of all pair combinations (the naive approach).
\paragraph{Expanding Multimodal Learning to Text} Our choice of a joint-embedding framework was deliberate, with future extensions in mind—in particular, the generalization of a $n>2$ multimodal training with the integration of unstructured text data, such as clinical notes, which are available in MIMIC-IV dataset. This rich textual information could further improve classification performance and enable the generation of more natural, text-based explanations for the model's predictions. We plan to generalize the joint-embedding objective to align representations from all three modalities (ECG, tabular, text). Crucially, we propose using the ECG's latent space as a central anchor, aligning the other modalities to it. This \emph{anchor-based} approach, inspired by the teacher-student approach in some SSL methods, is hypothesized to scale more effectively than the naive alternative of optimizing all pairwise combinations of modalities.

% \paragraph{conclusion} conclude the text, highlighting (i) the joint-embedding as a way to distill knowledge from other modes of data while keeping the ability to inference with just one of these; (ii) the other-mode prediction as a better way to explain the classification prediction in comparison to heatmaps in the input space


==> short/method.tex <==
\section{Method}
Our approach is a three-stage training paradigm designed to create a powerful ECG representation aligned with clinically relevant outputs. We first pre-train a waveform encoder using a self-supervised, cross-modal objective to transfer knowledge from tabular clinical data. Subsequently, we fine-tune this encoder for two downstream relevant clinical tasks: a primary task of multi-label diagnosis classification \cite{strodthoff2024prospects}; and, a secondary task of laboratory values abnormality prediction \cite{alcaraz2024cardiolab}.

\subsection{Joint-embedding Pre-training}
% should describe the barlow twins setup, using the joint-embedding loss to distill the information from the tabular data into the signal encoder

% we encode both the signal $x$ and tabular data $m$ with encoders $\Phi_x$ and $\Phi_m$ to $h_x$ and $h_m$, then align a projection of their embeddings $z_x$ and $z_m$ with projectors $\Theta_x$ and $\Theta_m$ with the barlow twins loss function $J_{je}$, like equation \ref{eq:je}

The primary goal of our pre-training stage is to learn a signal encoder, $\Phi_x$, whose representations are enriched with the contextual information present in associated tabular clinical data. To achieve this, we frame the task as a self-supervised, joint-embedding problem where the model learns to align representations from these two distinct modalities.

For a given patient encounter, we have a raw ECG signal segment $x \in \mathbb{R}^{C \times L}$, where $C$ is the number of leads and $L$ is the sequence length, and a corresponding vector of tabular clinical data $m \in \mathbb{R}^{D}$, which includes demographics, vitals, and biometrics. The signal and tabular data are processed by their respective encoders, a powerful S4-based sequence model $\Phi_x$ \citep{strodthoff2024prospects} and a MLP $\Phi_m$. These backbones produce feature representations $h_x = \Phi_x(x)$ and $h_m = \Phi_m(m)$. Following the standard practice in self-supervised learning, these feature representations are then mapped into another embedding space using dedicated projector networks, $\Theta_x$ and $\Theta_m$, $z_x = \Theta_x(h_x)$ and $z_m = \Theta_m(h_m)$, $z_x, z_m \in \mathbb{R}^{E}$, where $E$ is the embedding dimension.

To align these embeddings without risking representational collapse, we employ the Barlow Twins loss function, $\mathcal{L}_{BT}$. This objective function does not rely on negative sampling and instead encourages the cross-correlation matrix computed between the embeddings $Z_x$ and $Z_m$ over a batch of $N$ samples to be close to the identity matrix. The loss is composed of two terms: an invariance term that pulls the embeddings from the same patient together; and, a redundancy reduction term that decorrelates the different dimensions of the embedding vectors. The total pre-training objective is thus defined as in Equation~\ref{eq:je}.

\begin{equation}
\label{eq:je}
\mathcal{L}_{je} = \mathcal{L}_{BT}(Z_x, Z_m) = \sum_{i} (1 - C_{ii})^2 + \lambda \sum_{i} \sum_{j \neq i} C_{ij}^2
\end{equation}

where $C$ is the cross-correlation matrix computed between the batch-normalized embeddings $Z_x$ and $Z_m$, and $\lambda$ is a hyperparameter balancing the two terms. By minimizing this loss, the signal encoder $\Phi_x$ is trained to produce representations $h_x$ that are not only descriptive of the ECG signal itself but are also highly predictive of the rich, contextual information contained in the clinical data $m$. This process effectively transfers the clinical knowledge into the parameters of the waveform encoder.

\subsection{Diagnosis Classification}
% should describe the standard classification approach, i think we dont need to spend much space in this subsection

% we then finetune the signal encoder $\Phi_x$ to predict the diagnoses labels $y$ with a predictor $\Psi_y$ and train with bce loss function $\mathcal{L}_{BCE}$

Following the self-supervised pre-training stage, we leverage the learned, context-aware signal encoder $\Phi_x$ for the primary downstream task of clinical diagnosis prediction. To accomplish this, we adopt a standard fine-tuning protocol.

The pre-trained encoder $\Phi_x$ is partially frozen to prevent catastrophic forgetting of the transferred clinical knowledge. A new, task-specific classification head, $\Psi_y$, is then initialized and attached to the encoder. This head is a lightweight MLP that takes the feature representation $h_x = \Phi_x(x)$ and maps it to a logit for each of the $K$ possible diagnoses.

The model is then trained on the subset of the data containing ground-truth diagnosis labels $Y$. The optimization objective is the standard Binary Cross-Entropy (BCE) loss, summed over all possible labels, as is common for multi-label classification problems. The classification loss is defined as in Equation~\ref{eq:bce}.

\begin{equation}
\label{eq:bce}
\mathcal{L}_{c} = \mathcal{L}_{BCE}(Y, \hat{Y}) = -K^{-1} \sum_k^K [Y_k \log(\hat{Y}_k) + (1 - Y_k) \log(1 - \hat{Y}_k)]
\end{equation}

where $Y \in \{0, 1\}^K$ is the one-hot encoded vector of true labels and $\hat{Y}$ is the vector of predicted logits from the model. This fine-tuning stage adapts the powerful, general-purpose representation learned during pre-training to the specific patterns required for the diagnostic task.

\subsection{Reconstruction Finetuning}
% should describe the estimation task, predicting abnormalities of some features of the tabular data (laboratory exam related)

% we then use this signal encoder $\Phi_x$ for the reconstruction task, we want to use this prediction $\hat{m}^*$ as a way to explain the classification task, note however that we are not completed reconstructing the data $m$ but instead predicting a logit to identify abnormalities in some lab exam features (estimation task), in this context $m^*$ represents the one-hot encoding space of the abnormalities. we use another predictor $\Psi_m$ and train with bce loss function $\mathcal{L}_{BCE}$

A primary motivation for our three-stage approach is to produce a waveform representation that is not only predictive but also interpretable. We train the signal encoder $\Phi_x$ to perform a reconstruction task of laboratory abnormalities that are related to the context seem in the pre-training.

For this purpose, we introduce a second, independent head $\Psi_m$, which is attached to the same pre-trained encoder $\Phi_x$. This head is trained to predict a multi-label vector $M^* \in \{0, 1\}^P$, where $P$ is the number of distinct laboratory abnormalities defined in our dataset (e.g., "Hemoglobin\_high", "Urea Nitrogen\_low"). Each element $m^*_p \in M^*$ is a binary indicator of a specific lab abnormality.

Similar to the classification phase, the reconstruction head $\Psi_m$ is a lightweight MLP that takes the signal representation $h_x$ and outputs a vector of logits $\hat{M}^* = \Psi_m(\Phi_x(x))$, one for each of the $P$ lab abnormalities. The model is trained by minimizing the BCE loss, as defined in Equation~\ref{eq:bce}, now applied to the lab abnormality targets $m^*$ as in Equation~\ref{eq:recon}.

\begin{equation}
\label{eq:recon}
\mathcal{L}_{r} = \mathcal{L}_{BCE}(M^*, \hat{M}^*)
\end{equation}

The ability of the model to successfully perform this pseudo-reconstruction task, using only the ECG signal as input, serves to provide a mechanism for model explainability. For any given diagnosis prediction, we can now also output the concurrent lab abnormalities predicted from the same ECG embedding, offering clinicians a direct, data-driven insight into the potential physiological drivers behind the model's primary prediction. Essentially we offer something like: "The model predicts diagnosis $Y$, and it's doing so as it also is predicting a associated lab abnormality $M^*_p$ (e.g., high creatinine)."

